Groupwise Query Specialization and Quality-Aware Multi-Assignment for Transformer-based Visual Relationship Detection

Visual Relationship Detection (VRD) has seen significant advancements with Transformer-based architectures recently. However, we identify two key limitations in a conventional label assignment for training Transformer-based VRD models, which is a process of mapping a ground-truth (GT) to a prediction. Under the conventional assignment, an unspecialized query is trained since a query is expected to detect every relation, which makes it difficult for a query to specialize in specific relations. Furthermore, a query is also insufficiently trained since a GT is assigned only to a single prediction, therefore near-correct or even correct predictions are suppressed by being assigned no relation as a GT. To address these issues, we propose Groupwise Query Specialization and Quality-Aware Multi-Assignment (SpeaQ). Groupwise Query Specialization trains a specialized query by dividing queries and relations into disjoint groups and directing a query in a specific query group solely toward relations in the corresponding relation group. Quality-Aware Multi-Assignment further facilitates the training by assigning a GT to multiple predictions that are significantly close to a GT in terms of a subject, an object, and the relation in between. Experimental results and analyses show that SpeaQ effectively trains specialized queries, which better utilize the capacity of a model, resulting in consistent performance gains with zero additional inference cost across multiple VRD models and benchmarks. Code is available at https://github.com/mlvlab/SpeaQ.

==> tab_fig_tex/frequency_plot.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=0.9\linewidth]{figure/frequency_plot.pdf}    
\caption{\textbf{Prediction frequency of predicates in log-scale.}} 
\end{figure}


==> tab_fig_tex/group_assignment_fig.tex <==
\begin{figure}[t!]
\centering

\begin{minipage}{0.8\linewidth}
\begin{minipage}{0.48\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figure/ours_assign.pdf}
    \subcaption{\scriptsize \textbf{Prediction frequency} per group. The closer to the GT, the better.}
\end{minipage}
\hfill
\begin{minipage}{0.48\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figure/base_assign.pdf}
    \subcaption{\scriptsize \textbf{mR@100} per group. The higher, the better.}
\end{minipage}
\vspace{-0.2cm}
\caption{\small \textbf{Prediction frequency and mR@100} per group. Group 1 consists of the most frequent predicates, while group 5 consists of the least frequent predicates.}
\vspace{-0.5cm}
\end{minipage}
% \end{minipage}
\label{fig:training_signal_per_query}
\end{figure}

